Revisiting Depth Completion from a Stereo Matching Perspective for Cross-domain Generalization

This paper proposes a new framework for depth completion robust against domain-shifting issues. It exploits the generalization capability of modern stereo networks to face depth completion, by processing fictitious stereo pairs obtained through a virtual pattern projection paradigm. Any stereo network or traditional stereo matcher can be seamlessly plugged into our framework, allowing for the deployment of a virtual stereo setup that is future-proof against advancement in the stereo field. Exhaustive experiments on cross-domain generalization support our claims. Hence, we argue that our framework can help depth completion to reach new deployment scenarios.

==> preamble.tex <==
\usepackage[dvipsnames]{xcolor}
\usepackage{tabu}
\usepackage{amssymb}
\usepackage{pifont}
\usepackage{color, colortbl}


\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}

\DeclareCaptionFormat{teaser}{
    \textbf{#1#2}#3
}

\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
